Variational framework for partially-measured physical system control: examples of vision neuroscience and optical random media

To characterize a physical system to behave as desired, either its underlying governing rules must be known a priori or the system itself be accurately measured. The complexity of full measurements of the system scales with its size. When exposed to real-world conditions, such as perturbations or time-varying settings, the system calibrated for a fixed working condition might require non-trivial re-calibration, a process that could be prohibitively expensive, inefficient and impractical for real-world use cases. In this work, we propose a learning procedure to obtain a desired target output from a physical system. We use Variational Auto-Encoders (VAE) to provide a generative model of the system function and use this model to obtain the required input of the system that produces the target output. We showcase the applicability of our method for two datasets in optical physics and neuroscience.

==> Questions.tex <==
1.	For all authors...\\

(a) Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
	\textbf{\textbf{Response}}: Yes, please refer to Results section.
\\
\\
	 (b) Have you read the ethics review guidelines and ensured that your paper conforms to them?
	 \textbf{Response}: Yes.
\\	
\\	
	 (c) Did you discuss any potential negative societal impacts of your work?
 \textbf{Response}: Yes, please refer to the discussion and conclusion section.
\\
\\
	 (d) Did you describe the limitations of your work?
\textbf{Response}: Yes, please refer to the discussion and conclusion section.
\\
\\
2.	If you are including theoretical results...
(a) Did you state the full set of assumptions of all theoretical results?	\textbf{Response}: n/a
\\	
\\
	 (b) Did you include complete proofs of all theoretical results?
	\textbf{Response}: n/a
\\
\\
3.	If you ran experiments...
	(a) Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
	\textbf{Response}: Yes, please refer to the supplementary section.
\\
\\
	 (b) Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
	\textbf{Response}: Yes, please refer to the supplementary section.
\\
\\
 (c) Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
\textbf{Response}: Yes, please refer to Fig. 1.
\\
\\
	 (d) Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
	\textbf{Response}: Yes, please refer to the supplementary section.
\\
\\
4.	If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	(a) If your work uses existing assets, did you cite the creators?
	\textbf{Response}: Yes, please refer to the results section.
\\
\\
 (b) Did you mention the license of the assets?
\textbf{Response}: No. License is not required for usage or is data is publicly available.
\\
\\
	 (c) Did you include any new assets either in the supplemental material or as a URL?
	\textbf{Response}: Yes, assets are provided in the submission material and will be made public ally available upon publication.
\\
\\
 (d) Did you discuss whether and how consent was obtained from people whose data you're using/curating?
	\textbf{Response}: n/a
\\
\\
	 (e) Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
	\textbf{Response}: n/a
\\
\\
5.	If you used crowdsourcing or conducted research with human subjects...
	(a) Did you include the full text of instructions given to participants and screenshots, if applicable?
	\textbf{Response}: n/a
\\
\\
	 (b) Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
	\textbf{Response}: n/a
\\
\\
	 (c) Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
	\textbf{Response}: n/a

